Three-Polarizer Treatment of Linear Polarization in Coronagraphs and Heliospheric Imagers

Linear polarized light has been used to view the solar corona for over 150 years. While the familiar Stokes representation for polarimetry is complete, it is best matched to a laboratory setting and therefore is not the most convenient representation either for coronal instrument design or for coronal data analysis. Over the last 100 years of development of coronagraphs and heliospheric imagers, various representations have been used both for direct measurement and analysis. These systems include famous representations such as the (B, pB) system that is analogous to the Stokes system in solar observing coordinates, and also internal representations such as in-instrument Stokes parameters with fixed or variable "vertical" direction, and brightness values through a particular polarizing optic or set thereof. Many polarimetric instruments currently use a symmetric three-polarizer measurement and representation system, which we refer to as "(M, Z, P)", to derive the (B, pB) or Stokes parameters. We present a symmetric derivation of (B, pB) and Stokes parameters from (M, Z, P), analyze the noise properties of (M, Z, P) in the context of instrument design, develop (M, Z, P) as a useful intermediate system for data analysis including background subtraction, and draw a helpful analogy between linear polarimetric systems and the large existing body of work on photometric colorimetry.

==> litsearch.tex <==


- Howard & Tappin (2009): revisits the first-order theory of Thomson scattering, Van de Hulst coefficients, etc. Treats "degree of polarization" in the new sense (Equation 39)
- deKoning_Pizzo 2011: new-school (equation 7)

- Dai et al. 2014: nice review; use Ip=Bt-Br; eschews "pB" altogether

- Altschuler & Perry 1972: description of K coronameter; Equation 15: p=(It-Ir)/(It+Ir)  -- QUOTE THIS IN OUR DEFINITIONS

- Hayes Etal 2001: defines pB=Bt-Br
- DeForest et al. 2013: treat polarization following Altschuler & Perry
- Moran & Davila 2004: CME localiation; analysis uses Ip = It-Ir (their Equation 3)



- Bemporad et al. 2015: analysis of errors in CME location; mention pB as "total polarization"; use pB as quasi-Stokes (Equation 1)
- Guhathakurta et al. 1999: (coronal hole during WSM) - compares Mk III coronameter with SOHO/LASCO/C2.  "pB" used without explanation; implies two separate uses
- Frazin et al 2012: intercomparison mixes pB styles without comment



- Dere et al. 2005: LASCO polarization analysis; agrees with referee (p = (Q^2+U^2)^0.5 / I).  They call out polarizations within LASCO due to internal reflections;  this could be discussed in the error discussion.
- Ohman 1947: uses as total polarizsation (old school): their equation 19
- Billings 1966: develops "I_P" as sqrt(Q^2+U^2) (Equation 32, p. 98) but does not directly reference "pB".
- Munro & Jackson (1977): old-school
- Vorobiev et al. 2014: instrument paper uses "p = sqrt(Q^2+U^2+V^2)/I"
- Kohl et al. 1995: UVCS polarimeter channel agrees with referee (old school)

- Reginald et al. 2017: recent paper uses old school "pB" (cited by referee)

